Searches for Non-Standard Neutrino Oscillations with the IceCube Neutrino Observatory

The short-baseline neutrino anomalies observed by LSND, MiniBooNE, and the gallium experiments can be explained by additional neutrino states beyond the three established by solar, atmospheric, and reactor oscillation measurements. The minimal 3+1 sterile neutrino model that parameterizes these anomalies is in significant tension with null results from other oscillation experiments and with cosmological constraints, motivating the exploration of non-minimal extensions in which the additional mass eigenstate is unstable. This thesis presents a search for an unstable sterile neutrino model, in which the heavy mass eigenstate $\nu_4$ decays to two invisible particles, using 10.67 years of high-energy atmospheric neutrino data from the IceCube Neutrino Observatory. The analysis finds no preference for sterile decay over the no-decay 3+1 hypothesis and excludes most of the parameter space preferred by global fits to short-baseline data at 90% confidence level, providing a strong constraint on this non-minimal explanation of the anomalies. The thesis additionally develops the foundation for a future sterile neutrino search at IceCube targeting the resonant disappearance of antineutrinos. Three contributions are presented: a comprehensive calculation of neutrino-nucleon and neutrino-nucleus deep-inelastic scattering cross sections, new machine-learning reconstruction techniques, and an improved event selection with twice the signal efficiency of the previous iteration. Together, these tools enable statistical separation of neutrinos and antineutrinos and establish the infrastructure for the next generation of sterile neutrino searches with IceCube.

==> appendices/appa.tex <==



==> contents.tex <==
  % -*- Mode:TeX -*-
%% This file simply contains the commands that actually generate the table of
%% contents and lists of figures and tables.  You can omit any or all of
%% these files by simply taking out the appropriate command.  For more
%% information on these files, see appendix C.3.3 of the LaTeX manual. 
\tableofcontents
\newpage
\listoffigures
\newpage
\listoftables



==> cover.tex <==
% -*-latex-*-
% 
% For questions, comments, concerns or complaints:
% thesis@mit.edu
% 
%
% $Log: cover.tex,v $
% Revision 1.9  2019/08/06 14:18:15  cmalin
% Replaced sample content with non-specific text.
%
% Revision 1.8  2008/05/13 15:02:15  jdreed
% Degree month is June, not May.  Added note about prevdegrees.
% Arthur Smith's title updated
%
% Revision 1.7  2001/02/08 18:53:16  boojum
% changed some \newpages to \cleardoublepages
%
% Revision 1.6  1999/10/21 14:49:31  boojum
% changed comment referring to documentstyle
%
% Revision 1.5  1999/10/21 14:39:04  boojum
% *** empty log message ***
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.4  1997/04/18  17:54:10  othomas
% added page numbers on abstract and cover, and made 1 abstract
% page the default rather than 2.  (anne hunter tells me this
% is the new institute standard.)
%
% Revision 1.3  93/05/17  17:06:29  starflt
% Added acknowledgements section (suggested by tompalka)
% 
% Revision 1.2  92/04/22  13:13:13  epeisach
% Fixes for 1991 course 6 requirements
% Phrase "and to grant others the right to do so" has been added to 
% permission clause
% Second copy of abstract is not counted as separate pages so numbering works
% out
% 
% Revision 1.1  92/04/22  13:08:20  epeisach

% NOTE:
% These templates make an effort to conform to the MIT Thesis specifications,
% however the specifications can change. We recommend that you verify the
% layout of your title page with your thesis advisor and/or the MIT 
% Libraries before printing your final copy.
\title{Searches for Non-Standard Neutrino Oscillations\\
with The IceCube Neutrino Observatory}

\author{Philip Lawrence Rudolf Weigel}
% If you wish to list your previous degrees on the cover page, use the 
% previous degrees command:
%       \prevdegrees{A.A., Harvard University (1985)}
% You can use the \\ command to list multiple previous degrees
\prevdegrees{B.S., Drexel University (2020)}
\department{Department of Physics}

% If the thesis is for two degrees simultaneously, list them both
% separated by \and like this:
\degree{Doctor of Philosophy in Physics}
% \degree{Bachelor of Science in Computer Science and Engineering}

% As of the 2007-08 academic year, valid degree months are September, 
% February, or June.  The default is June.
\degreemonth{May}
\degreeyear{2026}
\thesisdate{May 6, 2026}

%% By default, the thesis will be copyrighted to MIT.  If you need to copyright
%% the thesis to yourself, just specify the `vi' documentclass option.  If for
%% some reason you want to exactly specify the copyright notice text, you can
%% use the \copyrightnoticetext command.  
%\copyrightnoticetext{\copyright IBM, 1990.  Do not open till Xmas.}

% If there is more than one supervisor, use the \supervisor command
% once for each.
\supervisor{Janet Conrad}{Professor}

% This is the department committee chairman, not the thesis committee
% chairman.  You should replace this with your Department's Committee
% Chairman.
\chairman{Scott Hughes}{Interim Associate Department Head}

% Make the titlepage based on the above information.  If you need
% something special and can't use the standard form, you can specify
% the exact text of the titlepage yourself.  Put it in a titlepage
% environment and leave blank lines where you want vertical space.
% The spaces will be adjusted to fill the entire page.  The dotted
% lines for the signatures are made with the \signature command.
\maketitle

% The abstractpage environment sets up everything on the page except
% the text itself.  The title and other header material are put at the
% top of the page, and the supervisors are listed at the bottom.  A
% new page is begun both before and after.  Of course, an abstract may
% be more than one page itself.  If you need more control over the
% format of the page, you can use the abstract environment, which puts
% the word "Abstract" at the beginning and single spaces its text.

%% You can either \input (*not* \include) your abstract file, or you can put
%% the text of the abstract directly between the \begin{abstractpage} and
%% \end{abstractpage} commands.

% First copy: start a new page, and save the page number.
\cleardoublepage
% Uncomment the next line if you do NOT want a page number on your
% abstract and acknowledgments pages.
% \pagestyle{empty}
\setcounter{savepage}{\thepage}
\begin{abstractpage}
\input{abstract}
\end{abstractpage}

% Additional copy: start a new page, and reset the page number.  This way,
% the second copy of the abstract is not counted as separate pages.
% Uncomment the next 6 lines if you need two copies of the abstract
% page.
% \setcounter{page}{\thesavepage}
% \begin{abstractpage}
% \input{abstract}
% \end{abstractpage}

\cleardoublepage

\section*{Acknowledgments}

I am deeply grateful to my advisor, Janet Conrad. I first started working with Janet in 2017 as a co-op on IsoDAR and returned in 2019 to continue, before beginning graduate school on IceCube in 2020.
She kept inviting me back, so I must have been doing something right. 
Throughout my time as a graduate student, she has taught me almost everything I know about being a good experimentalist and has given me ample intellectual freedom along the way.

Many people shaped my path toward physics. 
John Metroke and Jay Werkheiser fostered my interest in electrical engineering and physics in high school. 
Michelle Dolinski, who introduced me to neutrino physics and detector R\&D in my first year at Drexel, is solely responsible for converting me from engineering to physics. 
The real rigor of my hands-on training came from Dan Akerib at SLAC and Daniel Winklehner at MIT, from whom I learned a great deal about hardware and how to build experiments.

I would like to thank the graduate students of my group, past and present: Marjon, Alex, Joe, Loyd, Nick K., Darcy, Josh, Julia, and Claire; and the postdocs: Daniel, Austin, John H., Jarrett, and David. 
Everyone in the Harvard group has been a steady source of interesting ideas and discussions.
Spencer and Miles from the University of Delaware group helped me significantly with several parts of the new MEOWS event selection, and are my go-to contacts for calibration-related topics.

I have had many friends who have supported me along the way.
In particular, I would like to thank the core crew: Neil, John Walters, and Aidan, who have been a constant throughout these years.
Prairie Yang gets a special mention, of course.
Many of my friends from Drexel: Alan, Bassem, Brian, Dan$^2$, Nick, Huang, John B., Kar, and Shipper, were indispensable for getting through the COVID times and the lockdown boredom.
In the past year, Owen Jacob, Kyle, Emily, Josh, Igor, Jon, and Preston have been a source of never-ending fun and the closest thing one can call a ``social life'' while finishing up graduate school.

Lastly, I would like to thank Marina for her love and being my biggest supporter throughout these years.
Without her, I doubt I would be where I am today.


==> fontsets/mitthesis-defaultfonts.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-defaultfonts.tex}[2026/01/31 v1.07 Load Computer/Latin Modern text and math fonts]

%% Default fonts
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Computer Modern text and math fonts (default for pdftex)}
	\RequirePackage[T1]{fontenc} % With T1 encoding, pdftex will silently load the cm-super fontset
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
	\RequirePackage{bm}
	%
	\RequirePackage{etoolbox} % may already be loaded by the .cls file
	% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
	\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\else
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts (default for unicode engines)}
	%
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-fira-newtxsf.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-fira-newtxsf.tex}[2026/01/31 v1.07 Load Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font]

%% Adjusted sizes of text, math, and typewriter fonts, 2024/10/11
%% Fira Sans text font with newtx sans serif math font and Inconsolata typewriter font
%
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Fira sans text font with newtx sans serif math font and Inconsolata typewriter}
	\RequirePackage[U,T1]{fontenc}
    \RequirePackage[varqu,varl]{zi4} % inconsolata font for typewriter
    \RequirePackage[sfdefault,tabular,lf]{FiraSans} % sans serif text package
    % Use option lf to get lining figures rather than default, old style figures. Use tabular to get tabular figures, not proportional figures.
    % Best choice will vary, depending on what type of content you have. With some effort, these settings can be changed according to content,
    % See, e.g.: https://tex.stackexchange.com/q/114331/119566
    \renewcommand\rmdefault{\fira@family} % roman font for math (e.g., for operators) and for \textrm{..}
    \RequirePackage[scaled=1.1]{newtxsf}  % sans serif math; [noSTIXops] option suppresses STIX figures in favor of text font figures, 
    % in the most recent versions of newtxsf, but using the following for backward compatibility. NB: 'figures' means numbers: 0123456789.
    % This matters, for example, in tables that mix text and math figures.
        \DeclareSymbolFont{mynumbers}{T1}{FiraSans-TLF}{m}{n}
        \DeclareMathSymbol{0}{\mathord}{mynumbers}{`0}
        \DeclareMathSymbol{1}{\mathord}{mynumbers}{`1}
        \DeclareMathSymbol{2}{\mathord}{mynumbers}{`2}
        \DeclareMathSymbol{3}{\mathord}{mynumbers}{`3}
        \DeclareMathSymbol{4}{\mathord}{mynumbers}{`4}
        \DeclareMathSymbol{5}{\mathord}{mynumbers}{`5}
        \DeclareMathSymbol{6}{\mathord}{mynumbers}{`6}
        \DeclareMathSymbol{7}{\mathord}{mynumbers}{`7}
        \DeclareMathSymbol{8}{\mathord}{mynumbers}{`8}
        \DeclareMathSymbol{9}{\mathord}{mynumbers}{`9}
 	\RequirePackage{bm}
	%
	\RequirePackage{etoolbox} % may already be loaded by the .cls file
	% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
	\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\else
	\ClassWarning{\ClassName}{The fira-newtxsf font set requires pdflatex. Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-heros-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-heros-stix2.tex}[2025/10/23 v1.08 Load TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font]

%% TeX Gyre Heros (sans serif) text font with STIX Two Math font and Inconsolata monospaced font
%
%	These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%	They are also available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
%
\ifpdftex
	\ClassError{\ClassName}{The heros-stix2 fontset requires a unicode engine. Defaulting to CMR fonts}{To use the class option [fontset=heros-stix2] you must use a unicode engine, such as LuaLaTeX.}
	\RequirePackage[T1]{fontenc}
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{TeX Gyre Heros (sans serif) text font with STIX2 math font and Inconsolata monospaced font}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    \setmainfont{texgyreheros}[
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
    \setsansfont{texgyreheros}[
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,
	]        
   \setmonofont{Inconsolatazi4}[
        Scale=1.04,
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02}, % drop +ss03 (upright quotes), 2025/04/18
    ]             
    \setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes helpful
    	Scale=MatchLowercase,%0.95,%MatchUppercase,%MatchLowercase,
		% scaling is a matter of taste ... the x-heights of STIX2 are greater than for Heros...
    	Extension = .otf,
%		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
    ]
    % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
    %    
    \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Heros bold, https://github.com/stipub/stixfonts
    \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
    \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX Two
     %         
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-libertinus.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-libertinus.tex}[2025/09/23 v1.02 Load Libertinus and related fonts]

%% Libertinus (serif) text font with newtxmath[libertinus] (pdftex) or Libertinus (unicode) math font
%
%	These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%	They are also available at: 
%  		https://ctan.org/tex-archive/fonts/libertine/opentype 
%		https://github.com/alerque/libertinus
%
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Libertinus type1 text fonts and newtx-libertinus math fonts}
    \RequirePackage[T1]{fontenc}
    \RequirePackage[lf,t,semibold,ScaleTT=0.9]{libertinus} % tabular lining figures
    \RequirePackage[libertinus,vvarbb,subscriptcorrection]{newtxmath}% see package documentation for options
    \RequirePackage{bm}% load after all math to give access to bold math
\else
	\ClassNoteNoLine{\ClassName}{Loading Libertinus OTF text and math fonts}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode math loads the fontspec package
 	%
    \setmainfont{LibertinusSerif}[% 
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Semibold, 
    	BoldItalicFont = *-SemiboldItalic,
    	RawFeature={+ss05,+dlig,+tnum,+liga}, 
		% +ss02 would change J, K, R; +ss05 changes W; onum = oldstyle figures; hlig = historical ligatures
    ]    
    \setsansfont{LibertinusSans}[% 
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
	    BoldItalicFont = *-Bold,% does not have bold italic
    	Scale=MatchUppercase,
		RawFeature={+liga,},
	]
	%
    \setmonofont{LibertinusMono}[% 
    	Scale=0.9,% 2024/10/13
	    Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Regular,% does not have italic
    	BoldFont = *-Regular,% does not have bold 
	    BoldItalicFont = *-Regular,% does not have bold italic
	] 
	% 
	\newfontfamily\LibertinusDisplay{LibertinusSerifDisplay-Regular.otf}% a display font, as for titles
	%
	\newfontfamily\LibertinusInitials{LibertinusSerifInitials-Regular.otf}% Large initial letters, as for first word in chapter
	%	     	
    %% a Libertinus math font
    \setmathfont{libertinusmath-regular}[%
     	Extension = .otf,   
    	Scale=MatchUppercase,
%		BoldFont = *,% This font lacks a bold version; you could use FakeBold as a stand in
    	RawFeature={+ss08},% +ss08 gives slanted integrals (no other features) 	
    	]
	\setmathfont{Latin Modern Math}[range=\nabla,Scale=0.91] % I hate the backward nabla in Libertinus Math...
	
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-lmodern.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-lmodern.tex}[2025/09/23 v1.01 Load Latin Modern text and math fonts]

%% Default fonts
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts}
	\RequirePackage[T1]{fontenc}
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
	\RequirePackage{lmodern}
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts (default for unicode engines)}
	%
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi


==> fontsets/mitthesis-lucida.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-lucida.tex}[2026/01/31 v1.06 Load Lucida fonts]

%% Lucida Bright and Lucida Bright Math fonts (available from the TeX Users Group)

\ClassNoteNoLine{\ClassName}{Lucida Bright and Lucida Bright Math fonts}

\ifpdftex
	\RequirePackage[LY1]{fontenc}
	\RequirePackage[expert,vargreek,altbullet]{lucidabr}   % switch text and math fonts 
	% some other options: seriftt (much larger quad size!), lucidasmallscale % 2024/10/13
	\RequirePackage{bm}
\else
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package

    % FEATURE 	DESCRIPTION 											DEFAULT
    % dlig 		discretionary ligatures (f-ligatures in typewriter fnt) off
    % liga 		standard ligatures (f-ligatures, not monospaced fonts) 	on
    % onum 		old style numbers (Lucida Bright only)					off
    % smcp 		small caps 	(Lucida Bright, upright only)				off
    % zero 		slashed zero (sans and monospaced fonts)				off
    % locl 		script/language specific (localized) forms 				on
    %
    % FEATURE 	FONT 						DESCRIPTION
    % ss01 		Lucida Sans & Typewriter 	use dotted zero: 𝟶 vs. default 0.
    % ss01 		use Lucida-standard shapes:
    % 			Lucida Grande Mono 			ØOQ vs. default 0OQ;
    % 			Lucida Console 				ØOQ vs. default 0OQ.
    
    \setmainfont{LucidaBrightOT}[% main rm
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
    %     BoldItalicFeatures={Color=Purple4}, % fixed 2024/10/13
    %     UprightFeatures={Color=Salmon3},
    	  Scale=0.93,% increased from 0.92, 2024/10/13
    %	  Numbers ={OldStyle}, 
      ]
    %
    \setsansfont{LucidaSansOT}[% main sans
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Italic,
          BoldFont=*-Demi,
    	  BoldItalicFont=*-DemiItalic,
    	  Scale=MatchUppercase,
      ]
    %
    \setmonofont{LucidaSansTypewriterOT}[% main typewriter
          Ligatures=TeX,
          Extension=.otf,
          UprightFont=*,
          ItalicFont=*-Oblique,
          BoldFont=*-Bold,
          BoldItalicFont=*-BoldOblique,
          Scale=MatchLowercase,% changed from MatchUppercase, 2024/10/13
      ]
    
    %% MATH FONTS
    %
    % ss01 	alternate Latin lower case math italic identical to text italic. This option is not recommended as Greek 𝜈 (nu) and Latin 𝑣 (vee) become too similar
    % ss02 	smaller arrows (original Type 1 size): ⇑ vs. default ⇑.
    % ss03 	attempt to imitate Type 1 fonts
    % ss04 	calligraphic alternative (similar to the Type 1 design) to the math script alphabet
    % ss05 	use a slashed-zero style for the empty set character (U+2205): Ø vs. default ∅
    % ss08 	emphasize right and bottom edges of the d’Alembertian operator (U+29E0, \laplac), to follow the design of the Laplace operator (U+2206, \increment, Δ); the default design emphasizes the left and upper edges. Also available in the bold math font.
    %
    \setmathfont{LucidaBrightMathOT}[% main math
    	  Scale=MatchUppercase,
    	  Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
%    	  BoldFeatures={Color=Chartreuse4},
    	  RawFeature ={+ss04,+ss08}, %
    ]
 
%% LucidaMath-OT contains a *serif* typerwriter font. If you prefer a sans serif typerwriter font, you can use the following two settings. 
% 
%    \setmathfont{LucidaSansTypewriterOT}[% <== NB: setting a text font where math font should go.
%    	  Scale=MatchUppercase,
%          range=tt,
%    	  Color=NavyBlue,
%          Extension=.otf,
%          script-features = {},     
%          sscript-features = {},     
%    	  BoldFont=LucidaSansTypewriterOT-Bold.otf,
%    	  BoldFeatures={Color=Salmon3},
%    ]
%    %
%    \setmathfontface\mathtt{LucidaSansTypewriterOT-Bold}[% bold upright typewriter font in boldmath.
%    	  version=bold,
%    	  Scale=MatchUppercase,
%          Extension=.otf,    
%    ]
	%
    \setmathfont{LucidaBrightMathOT}[%
    	  range={scr},% to make scr differ from cal
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,% could be overridden by bold separate version
    ]
    \setmathfont{LucidaBrightMathOT}[% -Demi .. sufficient this way, since bold set above.
    	  range={bfscr},% need to call \symbfscr manually - bug in unicode-math version & range interaction
    	  RawFeature={-ss04},
    	  Scale=MatchUppercase,
          Extension=.otf,
    	  BoldFont=LucidaBrightMathOT-Demi.otf,
    ]
    %% Fix unicode-math operator font not set up for bold face (default \mathrm). See https://github.com/wspr/unicode-math/issues/468
    \setoperatorfont\symup
    %
    % note \mathbfit = \symbfit
    
    % The specialized one-off Lucida fonts:
    \newfontface\LucidaBlackletter{LucidaBlackletterOT}[%
    	Scale=0.95,% <== NB
    	Extension=.otf,
    	]
    \newfontface\LucidaCalligraphy{LucidaCalligraphyOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
    	]
    \newfontface\LucidaHandwriting{LucidaHandwritingOT}[%
    	Scale=MatchUppercase,
    	Extension=.otf,
     	]
    % GrandeMono and Console fonts:
    \newfontface\LucidaGrandeMonoDK{LucidaGrandeMonoDK}[%	
    	Scale=MatchUppercase,
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
    \newfontface\LucidaConsole{LucidaConsoleDK}[%
    	Scale=MatchLowercase,% <=== NB
    	Extension=.otf,
        UprightFont=*,
        ItalicFont=*-Italic,
        BoldFont=*-Bold,
        BoldItalicFont=*-BoldItalic,
    	]
\fi
%
\RequirePackage{etoolbox} % may already be loaded by the .cls file
% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}


==> fontsets/mitthesis-newtx-sans-text.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx-sans-text.tex}[2026/01/31 v1.05 Load newtx sans-serif text and regular math fonts]

%% newtx package with sans-serif text (Helvetica-like text with Times-like math)
%
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading newtx sans-serif text and newtx serif math fonts}
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91,defaultsups]{newtx}% upint for upright integrals
	\AtEndPreamble{% added to accommodate v1.731 of newtx, 2023/11/03
	    \renewcommand{\familydefault}{\sfdefault}% use sans for main text
%	    \renewcommand{\rmdefault}{\sfdefault}% uses sans for \textrm{}, if that's desired.
	}
%   these two commands enable hyphenation of the typewriter font - https://tex.stackexchange.com/a/204421/119566
%    \input{t1ntxtt.fd}
%    \DeclareFontFamily{\encodingdefault}{\ttdefault}{\hyphenchar\font=`\-} % 
	\RequirePackage{bm}% bold math
	%
	\RequirePackage{etoolbox} % may already be loaded by the .cls file
	% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
	\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\else
	\ClassWarning{\ClassName}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> fontsets/mitthesis-newtx.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-newtx.tex}[2026/01/31 v1.05 Load newtx text and math fonts]

\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading newtx fonts with inconsolata typewriter}
	\RequirePackage[T1]{fontenc}
    \RequirePackage[subscriptcorrection,varvw,helvratio=0.91]{newtx}% stix2, upint
    \RequirePackage[varl,varqu,hyphenate,mono]{inconsolata}% sans typewriter font; mono = fixed word spacing, hyphenate = allow hyphenation 
	\RequirePackage{bm}
	\let\textsuperscript\textsu% newtx changes the default superiors font; this is needed to get commas aligned in sequential footnotes
	%
	\RequirePackage{etoolbox} % may already be loaded by the .cls file
	% Patch headings to automatically use \mathversion{bold}. Compare to report.cls. 
	\patchcmd{\section}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subsubsection}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\paragraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
	\patchcmd{\subparagraph}{\normalfont}{\mathversion{bold}\normalfont}{}{}
\else
	\ClassWarning{\ClassName}{The newtx font set requires pdflatex.  Defaulting to LMR fonts}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket}]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads the fontspec package, but the default fonts are not selected by fontspec in this case.
\fi

	

==> fontsets/mitthesis-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-stix2.tex}[2025/09/23 v1.08 Load STIX Two text and math fonts]

%% STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font
%
%	These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%	They are also available at: 
%				https://github.com/stipub/stixfonts 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://ctan.org/tex-archive/fonts/inconsolata
%
\ifpdftex
	\ClassError{\ClassName}{The stix2 fontset requires a unicode engine. Defaulting to CMR fonts.}{Use LuaLatex to run with the class option [fontset=stix2]}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading STIX Two text and math fonts with Heros sans serif font and Inconsolata monospaced font}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{STIXTwoText}[
       	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
	]
	\setsansfont{texgyreheros}[ 
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% 
	]        
	\setmonofont{Inconsolatazi4}[
        Scale=1.035,% 2024/10/13
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02}, % drop +ss03 (upright quotes), 2025/04/18
    ]             
	\setmathfont{STIXTwoMath-Regular}[
    	Scale=MatchUppercase,
    	Extension = .otf,
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes-stix2.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes-stix2.tex}[2025/09/23 v1.08 Load TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font]

%% TeX Gyre Termes text font and Heros sans serif font with STIX2 math font and Inconsolata monospaced font
%
%	These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%	They are also available at: 
%				http://www.gust.org.pl/projects/e-foundry/tex-gyre 
%				https://github.com/stipub/stixfonts 
%				https://ctan.org/tex-archive/fonts/inconsolata
%
\ifpdftex
	\ClassError{\ClassName}{The termes-stix2 fontset requires a unicode engine. Defaulting to CMR fonts}{To use the class option [fontset=termes-stix2], use a unicode engine such as LuaLaTeX.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading TeX Gyre Termes text font with STIX2 math font, Heros sans serif font, and Inconsolata monospaced font}
	%
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[
		WordSpace = {1,1.4,1},%% This stretch matches newtxtext a little better. 1.4
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
	\setsansfont{texgyreheros}[
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as for newtx; former value 0.9 too small 2022/01/15
	]        
	\setmonofont{Inconsolatazi4}[
        Scale=1,% reset to 1, 2024/10/12 %1.03,% rescaled from 1, 22/03/10
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Regular,% has no italic face
        BoldFont = *-Bold, 
    	BoldItalicFont = *-Bold,% has no bold italic face
        RawFeature = {+ss01,+ss02}, % drop +ss03 (upright quotes), 2025/04/18
    ]             
	\setmathfont{STIXTwoMath-Regular}[% nice glyphs, but \mkern sometimes helpful
    	Scale=MatchUppercase,
    	Extension = .otf,
%		BoldFont = *,% STIX Two Math has no bold face
%       Color=NavyBlue, 
    	RawFeature = {+ss01, -ss02, -ss08},
   ]
   % ss01 -- switch calligraphic to script; +ss02 -- variants of g, u, v, w, z; +ss08 -- upright integrals
   %
   \setmathfontface\mathbf{STIXTwoText-Bold.otf}[]% to not get Termes bold
   \setmathfontface\mathit{STIXTwoText-Italic.otf}[]
   \setmathfontface\mathrm{STIXTwoText-Regular.otf}[]% to get roman letters from STIX, not Termes
    %      
   \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2} 
\fi


==> fontsets/mitthesis-termes.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-termes.tex}[2025/09/23 v1.07 Load TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font]

%% TeX Gyre Termes (Times-like) text font with Termes math font and Heros sans serif font and Cursor monospaced font
%
%  These fonts are in TeX Live and on CTAN. They are included in a complete LaTeX installation. 
%  They are also available at: http://www.gust.org.pl/projects/e-foundry/tex-gyre
%
\ifpdftex
	\ClassError{\ClassName}{The termes fontset requires a unicode engine. Defaulting to CMR fonts}{To use the class option [fontset=termes], use a unicode engine such as LuaLaTeX.}
	\RequirePackage[T1]{fontenc}	
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading TeX Gyre Termes text and math fonts, Heros sans serif font, and Cursor monospaced font}
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math
    % unicode-math loads the fontspec package
	%
    \setmainfont{TeXGyreTermesX}[
		WordSpace = {1,1.4,1},
    	Extension = .otf,
    	UprightFont = *-Regular,
    	ItalicFont = *-Italic,
    	BoldFont = *-Bold,
    	BoldItalicFont = *-BoldItalic,
		SlantedFont = *-Italic,
		Numbers = Lining,
	]
    \setsansfont{texgyreheros}[
		WordSpace = {1,1.4,1},
		Extension = .otf,
    	UprightFont = *-regular,
    	ItalicFont = *-italic,
    	BoldFont = *-bold,
    	BoldItalicFont = *-bolditalic,
		Numbers = Lining,
    	Scale=0.91,% same as used in newtx; former value 0.9 too small 2022/01/15
	]        
   \setmonofont{texgyrecursor}[
        %Scale=0.97,
        Scale=1.03, % adjusted 2024/10/12 to bring x-size closer to other fonts
        Extension = .otf,
        UprightFont = *-Regular,
        ItalicFont = *-Italic,
        BoldFont = *-Bold, 
    	BoldItalicFont = *-BoldItalic,
%		BoldFeatures = { Color = VioletRed3 },
    ]             
    \setmathfont{texgyretermes-math}[
    	Scale=MatchUppercase,
    	Extension = .otf,
%		BoldFont = *, % termes-math does not have a bold version
%       Color=Red3, 
    ]
    %   
    \newcommand*{\FRAC}[1]{{\addfontfeature{Fractions=On}#1}}% use OpenType feature for fractions, \FRAC{1/2}
\fi


==> preamble.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{empheq}
\usepackage{cancel}
\usepackage{slashed}
\usepackage{yfonts}
\usepackage{float}
\usepackage{tikz}
\usepackage{physics}
\usepackage{pdfpages}
\usepackage{subcaption}
\usepackage{placeins}
\usepackage{enumitem}

\definecolor{linkcol}{RGB}{0,60,120}
\definecolor{citecol}{RGB}{0,100,50}
\definecolor{urlcol}{RGB}{120,0,60}

\usepackage[colorlinks=true,
            linkcolor=linkcol,
            citecolor=citecol,
            urlcolor=urlcol]{hyperref}
\usepackage[capitalize,noabbrev]{cleveref}
\usetikzlibrary{matrix,calc}

\newcommand\stoplabeling{\def\makelabel##1{}}
\newcommand\resumelabeling{\def\makelabel##1{\hss\llap{##1}}}
\newcommand{\He}{{^{3}\textrm{He}}}
\newcommand{\Lagr}{\mathcal{L}}
\newcommand{\nuSQuIDS}{nuSQuIDS}

